On the (Non-)Robustness of Two-Layer Neural Networks in Different Learning Regimes

Neural networks are known to be highly sensitive to adversarial examples. These may arise due to different factors, such as random initialization, or spurious correlations in the learning problem. To better understand these factors, we provide a precise study of the adversarial robustness in different scenarios, from initialization to the end of training in different regimes, as well as intermediate scenarios, where initialization still plays a role due to "lazy" training. We consider over-parameterized networks in high dimensions with quadratic targets and infinite samples. Our analysis allows us to identify new tradeoffs between approximation (as measured via test error) and robustness, whereby robustness can only get worse when test error improves, and vice versa. We also show how linearized lazy training regimes can worsen robustness, due to improperly scaled random initialization. Our theoretical results are illustrated with numerical experiments.

==> checklist.tex <==
\section*{Checklist}


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}: for each theorem, the conditions and hypothsesis under which they hold are clearly stated (see Conditions \ref{cond:growth}, \ref{cond:nonlinear}, \ref{cond:traces})
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}, we don't expect any.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}, refer to Section \ref{sec:prelim}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{} in the Appendix
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}, after every theoretical result, we provide empirical verification (e.g., see Figures \ref{fig:rf} and \ref{fig:allnt}). The code is given in a separate zip file.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNo{}, as our experiments have illustration purposes and are very simple.
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{}, as our experiments are very quick even on a basic setup (personal computer, no specific ressources).
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{}, as the MNIST dataset is widely used.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> general_lowerbound.tex <==


\section{A universal lower-bound}
\mytodo{Remove this section before submitting!}

Let $H^1(N(0,I_d))$ be the collection of functions $f:\mathbb R^d \to \mathbb R$ which are square-integrable w.r.t $N(0,I_d)$ and weakly-differentiable (in the sense Schwartz distributions), with derivative $\nabla f$ which is norm-square-integrable w.r.t $N(0,I_d)$.
\begin{restatable}[No Free Lunch]{thm}{}
For any $f \in L^1(N(0,I_d)) \cap H^1(N(0,I_d))$ with $\egen(f) \le E < 1$, it holds that
\begin{eqnarray}
\erob(f) \ge \frac{1}{4}(1-E^{1/2})^2.
\end{eqnarray}
\end{restatable}
This is a very general lower-bound which is independent of the structure of the model $f$ (neural network or not!).
\begin{proof}
Let $f \in L^1(N(0,I_d)) \cap H^1(N(0,I_d))$ and $\overline{f}$ be the mean value of $f$ w.r.t $N(0,I_d)$.
Applying the Poincar\'e inequality\footnote{e.g, see \url{https://hal.archives-ouvertes.fr/hal-01781502/file/guefi.pdf}.} for $N(0,I_d)$ gives
\begin{eqnarray*}
\begin{split}
\|\nabla f\|_{L^2(N(0,I_d))} \ge \|f-\overline{f}\|_{L^2(N(0,I_d))} &\ge \|f_\star-\overline{f}\|_{L^2(N(0,I_d))} - \|f-f_\star\|_{L^2(N(0,I_d))}\\
&\ge \|f_\star-\overline{f_\star}\|_{L^2(N(0,I_d))} - \|f-f_\star\|_{L^2(N(0,I_d))}\\
&= \|f_\star\|_{L^2(N(0,I_d))} - \|f-f_\star\|_{L^2(N(0,I_d))}\\
&= \|f_\star\|_{L^2(N(0,I_d))}\left(1-\frac{\|f-f_\star\|_{L^2(N(0,I_d))}}{\|f_\star\|_{L^2(N(0,I_d))}}\right).
\end{split}
\end{eqnarray*}
Squaring both sides, dividing by $\varepsilon_{\mathrm{test}}(f_\star) = 4\|f_\star\|^2_{L^2(N(0,1))}$, and recalling the definitions of $\egen(f)$ and $\erob(f)$ from Section \ref{subsec:metrics} then gives the result.
\end{proof}

==> table.tex <==
\begin{table*}[!ht]
  \begin{center}
       {\tabulinesep=1.2mm
    \begin{tabu}{c|c|c|c}
    \midrule
      Model $\mathcal M$ & Neurons per input dim $\rho$ &
      % Rescaled robustness 
      Relative nonrobustness &      Reference \\
      \midrule
      NN with SGD, quadratic activation & $0 < \rho < \infty$ & $\|B\|_{F,m}^2/\|B\|_F^2 \le 1$ & Theorem \ref{thm:sobsgd} \\
      \midrule
      RF, general activation $\sigma$ & $0 < \rho < \infty$ & $\dfrac{\tau^2(2\kappa\psi_1^2+\psi_2)}{\|B\|_F^2(2\kappa\psi_1 + 2)^2}$ & Theorem \ref{thm:rfratio} \\
    \midrule
      RF, general activation $\sigma$ & $\rho \to \infty$ & $\dfrac{\trace(B\Gamma)^2}{\|B\|_F^2\|\Gamma\|_F^2}\le 1$ & Theorem \ref{thm:rfratio} \\
    \midrule
      RF, general activation $\sigma$ & $0 < \rho < \infty$ & $\dfrac{\trace(B\Gamma)^2\|\Gamma\|_F^2m^2}{\|B\|_F^2(2+\|\Gamma\|_F^2m)^2}$ & Corollary \ref{cor:rfratio} \\
    \midrule
      RF, quadratic activation & $\rho \to \infty$ & $\dfrac{\trace(B\Gamma)^2}{\|B\|_F^2\|\Gamma\|_F^2}\le 1$ & Corollary \ref{cor:rfratio}\\
      \midrule
      NN at init, general activation $\sigma$ &  & $\dfrac{\|\sigma'\|^2_{L^2} + \lambda_3^2\|\Gamma\|_F^2/2 + \lambda_2^2\|\Gamma\|_F^2 }{4\|B\|_F^2}$ & Theorem \ref{thm:untrained} \\
      \midrule
      NN at init, quadratic activation &  & $(1+\|\Gamma\|_F^2)/\|B\|_F^2$ & Theorem \ref{thm:untrained} \\
      \midrule
        NT  w/o init term, quadratic activ. & $0 < \rho < \infty$ & $(\underline{\rho}+\underline{\rho}^2)/2+(\underline{\rho}-\underline{\rho})^2\trace(B)^2/(2d\|B\|_F^2)$ & Theorem \ref{thm:nt}\\
      \midrule
        NT  with init term, quadratic activ. & $0 < \rho < \infty$ & Sum of 2 previous rows & Theorem \ref{thm:ntl}\\
     % \midrule
    %   $\rf_{\text{init}}$ & $0 < \rho < \infty$ & $\ge \dfrac{m\|\Gamma\|_F}{\|B\|_F} \gtrsim m$ & Lm. \ref{lm:
    %   \midrule
    \end{tabu}
    }
  \end{center}
    \caption{Summary of main results. We compare the (non)robustness of a model $f_\mathcal M$
    % (for $\mathcal M \in \{\sgd,\rf,\rf_{\text{init}},\nt\}$)
    with that of the ground truth model $f_\star$ defined in \eqref{eq:truemodel}, as measured by the rescaled measure of nonrobustness $\widetilde{s}(f_{\mathcal M}):=\mathfrak{S}(f_{\mathcal M})^2/\mathfrak{S}(f_\star)^2$. Results are asymptotic with $m,d \to \infty$ such that $m/d \to \rho$ (refer to \eqref{eq:proportionate}). $\Gamma$ is the covariance matrix of the random features model at initialization.  % "Quadratic RF" is the random features model with quadratic activation function $\sigma(z) = z^2-1$.
    The positive scalars $\psi_1$ and $\psi_2$ are defined in \eqref{eq:psis}, and we define  $\underline{\rho} := \min(\rho,1)$. % $\Gamma$ is the covariance matrix of the random hidden weights matrix.
     }
    \label{Tab:main}
\end{table*}
